Cross-Process Defect Attribution using Potential Loss Analysis

Cross-process root-cause analysis of wafer defects is among the most critical yet challenging tasks in semiconductor manufacturing due to the heterogeneity and combinatorial nature of processes along the processing route. This paper presents a new framework for wafer defect root cause analysis, called Potential Loss Analysis (PLA), as a significant enhancement of the previously proposed partial trajectory regression approach. The PLA framework attributes observed high wafer defect densities to upstream processes by comparing the best possible outcomes generated by partial processing trajectories. We show that the task of identifying the best possible outcome can be reduced to solving a Bellman equation. Remarkably, the proposed framework can simultaneously solve the prediction problem for defect density as well as the attribution problem for defect scores. We demonstrate the effectiveness of the proposed framework using real wafer history data.

==> definitions.tex <==
\RequirePackage{todonotes}
\RequirePackage{latexsym}
\RequirePackage{amssymb}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{dsfont}
\RequirePackage{stmaryrd}
\RequirePackage{mathrsfs}
\RequirePackage{mathtools}
%\RequirePackage[capitalise]{cleveref}
\RequirePackage{ascmac}
\RequirePackage{comment}
\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{multicol}
\RequirePackage{nicematrix}

\newcommand{\ide}[1]{{\color{blue}#1}}

% Algorithm
% To use algorithm + algorithmicx, uncomment the following
% \RequirePackage{algorithm}
% \RequirePackage{algpseudocode}
% \renewcommand{\Return}{\textbf{return} }  % in case of conflicting with other package

% XXX: algorithm template
% \begin{algorithm}[tb]
%     \caption{test}
%     \label{alg:test}
%     \begin{algorithmic}[1]
% 
%         \Function {max\_in\_array}{$array$}
%         \State $max \gets 0$
%         \ForAll {$element \gets array$} 
%         \If {$element > max$}
%         \State $max \gets element$
%         \EndIf
%         \EndFor
%         % \State \textbf{return} $max$
%         \State \Return $max$
%         \EndFunction
% 
%     \end{algorithmic}
% \end{algorithm}


% Table
% ABCDEFGHIJKLMNOPQRSTUVWXYZ
% ell
% alpha beta gamma delta epsilon varepsilon eta iota kappa lambda mu nu pi rho sigma varsigma theta xi upsilon phi psi zeta omega 
% Gamma Delta Lambda Pi Sigma Theta Xi Upsilon Phi Psi Omega
\newcommand{\ellbar}{\bar{\ell}}
\newcommand{\ellhat}{\hat{\ell}}
\newcommand{\elltil}{\tilde{\ell}}

% bar shorthands
\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
% \newcommand{\hbar}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
% \newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}
\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}
\newcommand{\alphabar}{\bar{\alpha}}
\newcommand{\betabar}{\bar{\beta}}
\newcommand{\gammabar}{\bar{\gamma}}
\newcommand{\deltabar}{\bar{\delta}}
\newcommand{\epsilonbar}{\bar{\epsilon}}
\newcommand{\varepsilonbar}{\bar{\varepsilon}}
\newcommand{\etabar}{\bar{\eta}}
\newcommand{\iotabar}{\bar{\iota}}
\newcommand{\kappabar}{\bar{\kappa}}
\newcommand{\lambdabar}{\bar{\lambda}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\nubar}{\bar{\nu}}
\newcommand{\pibar}{\bar{\pi}}
\newcommand{\rhobar}{\bar{\rho}}
\newcommand{\sigmabar}{\bar{\sigma}}
\newcommand{\varsigmabar}{\bar{\varsigma}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\xibar}{\bar{\xi}}
\newcommand{\upsilonbar}{\bar{\upsilon}}
\newcommand{\phibar}{\bar{\phi}}
\newcommand{\psibar}{\bar{\psi}}
\newcommand{\zetabar}{\bar{\zeta}}
\newcommand{\omegabar}{\bar{\omega}}
\newcommand{\Gammabar}{\bar{\Gamma}}
\newcommand{\Deltabar}{\bar{\Delta}}
\newcommand{\Lambdabar}{\bar{\Lambda}}
\newcommand{\Pibar}{\bar{\Pi}}
\newcommand{\Sigmabar}{\bar{\Sigma}}
\newcommand{\Thetabar}{\bar{\Theta}}
\newcommand{\Xibar}{\bar{\Xi}}
\newcommand{\Upsilonbar}{\bar{\Upsilon}}
\newcommand{\Phibar}{\bar{\Phi}}
\newcommand{\Psibar}{\bar{\Psi}}
\newcommand{\Omegabar}{\bar{\Omega}}


% hat shorthands
\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}
\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\betahat}{\hat{\beta}}
\newcommand{\gammahat}{\hat{\gamma}}
\newcommand{\deltahat}{\hat{\delta}}
\newcommand{\epsilonhat}{\hat{\epsilon}}
\newcommand{\varepsilonhat}{\hat{\varepsilon}}
\newcommand{\etahat}{\hat{\eta}}
\newcommand{\iotahat}{\hat{\iota}}
\newcommand{\kappahat}{\hat{\kappa}}
\newcommand{\lambdahat}{\hat{\lambda}}
\newcommand{\muhat}{\hat{\mu}}
\newcommand{\nuhat}{\hat{\nu}}
\newcommand{\pihat}{\hat{\pi}}
\newcommand{\rhohat}{\hat{\rho}}
\newcommand{\sigmahat}{\hat{\sigma}}
\newcommand{\varsigmahat}{\hat{\varsigma}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\xihat}{\hat{\xi}}
\newcommand{\upsilonhat}{\hat{\upsilon}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\psihat}{\hat{\psi}}
\newcommand{\zetahat}{\hat{\zeta}}
\newcommand{\omegahat}{\hat{\omega}}
\newcommand{\Gammahat}{\hat{\Gamma}}
\newcommand{\Deltahat}{\hat{\Delta}}
\newcommand{\Lambdahat}{\hat{\Lambda}}
\newcommand{\Pihat}{\hat{\Pi}}
\newcommand{\Sigmahat}{\hat{\Sigma}}
\newcommand{\Thetahat}{\hat{\Theta}}
\newcommand{\Xihat}{\hat{\Xi}}
\newcommand{\Upsilonhat}{\hat{\Upsilon}}
\newcommand{\Phihat}{\hat{\Phi}}
\newcommand{\Psihat}{\hat{\Psi}}
\newcommand{\Omegahat}{\hat{\Omega}}

% tilde shorthands
\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}
\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\betatil}{\tilde{\beta}}
\newcommand{\gammatil}{\tilde{\gamma}}
\newcommand{\deltatil}{\tilde{\delta}}
\newcommand{\epsilontil}{\tilde{\epsilon}}
\newcommand{\varepsilontil}{\tilde{\varepsilon}}
\newcommand{\etatil}{\tilde{\eta}}
\newcommand{\iotatil}{\tilde{\iota}}
\newcommand{\kappatil}{\tilde{\kappa}}
\newcommand{\lambdatil}{\tilde{\lambda}}
\newcommand{\mutil}{\tilde{\mu}}
\newcommand{\nutil}{\tilde{\nu}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\rhotil}{\tilde{\rho}}
\newcommand{\sigmatil}{\tilde{\sigma}}
\newcommand{\varsigmatil}{\tilde{\varsigma}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\xitil}{\tilde{\xi}}
\newcommand{\upsilontil}{\tilde{\upsilon}}
\newcommand{\phitil}{\tilde{\phi}}
\newcommand{\psitil}{\tilde{\psi}}
\newcommand{\zetatil}{\tilde{\zeta}}
\newcommand{\omegatil}{\tilde{\omega}}
\newcommand{\Gammatil}{\tilde{\Gamma}}
\newcommand{\Deltatil}{\tilde{\Delta}}
\newcommand{\Lambdatil}{\tilde{\Lambda}}
\newcommand{\Pitil}{\tilde{\Pi}}
\newcommand{\Sigmatil}{\tilde{\Sigma}}
\newcommand{\Thetatil}{\tilde{\Theta}}
\newcommand{\Xitil}{\tilde{\Xi}}
\newcommand{\Upsilontil}{\tilde{\Upsilon}}
\newcommand{\Phitil}{\tilde{\Phi}}
\newcommand{\Psitil}{\tilde{\Psi}}
\newcommand{\Omegatil}{\tilde{\Omega}}

% bf shorthands
\newcommand{\abf}{\mathbf{a}}
\newcommand{\bbf}{\mathbf{b}}
\newcommand{\cbf}{\mathbf{c}}
\newcommand{\dbf}{\mathbf{d}}
\newcommand{\ebf}{\mathbf{e}}
\newcommand{\fbf}{\mathbf{f}}
\newcommand{\gbf}{\mathbf{g}}
\newcommand{\hbf}{\mathbf{h}}
\newcommand{\ibf}{\mathbf{i}}
\newcommand{\jbf}{\mathbf{j}}
\newcommand{\kbf}{\mathbf{k}}
\newcommand{\lbf}{\mathbf{l}}
\newcommand{\mbf}{\mathbf{m}}
\newcommand{\nbf}{\mathbf{n}}
\newcommand{\obf}{\mathbf{o}}
\newcommand{\pbf}{\mathbf{p}}
\newcommand{\qbf}{\mathbf{q}}
\newcommand{\rbf}{\mathbf{r}}
\newcommand{\sbf}{\mathbf{s}}
\newcommand{\tbf}{\mathbf{t}}
\newcommand{\ubf}{\mathbf{u}}
\newcommand{\vbf}{\mathbf{v}}
\newcommand{\wbf}{\mathbf{w}}
\newcommand{\xbf}{\mathbf{x}}
\newcommand{\ybf}{\mathbf{y}}
\newcommand{\zbf}{\mathbf{z}}
\newcommand{\Abf}{\mathbf{A}}
\newcommand{\Bbf}{\mathbf{B}}
\newcommand{\Cbf}{\mathbf{C}}
\newcommand{\Dbf}{\mathbf{D}}
\newcommand{\Ebf}{\mathbf{E}}
\newcommand{\Fbf}{\mathbf{F}}
\newcommand{\Gbf}{\mathbf{G}}
\newcommand{\Hbf}{\mathbf{H}}
\newcommand{\Ibf}{\mathbf{I}}
\newcommand{\Jbf}{\mathbf{J}}
\newcommand{\Kbf}{\mathbf{K}}
\newcommand{\Lbf}{\mathbf{L}}
\newcommand{\Mbf}{\mathbf{M}}
\newcommand{\Nbf}{\mathbf{N}}
\newcommand{\Obf}{\mathbf{O}}
\newcommand{\Pbf}{\mathbf{P}}
\newcommand{\Qbf}{\mathbf{Q}}
\newcommand{\Rbf}{\mathbf{R}}
\newcommand{\Sbf}{\mathbf{S}}
\newcommand{\Tbf}{\mathbf{T}}
\newcommand{\Ubf}{\mathbf{U}}
\newcommand{\Vbf}{\mathbf{V}}
\newcommand{\Wbf}{\mathbf{W}}
\newcommand{\Xbf}{\mathbf{X}}
\newcommand{\Ybf}{\mathbf{Y}}
\newcommand{\Zbf}{\mathbf{Z}}


% mathbb shorthands
\newcommand{\doubleA}{\mathbb{A}}
\newcommand{\doubleB}{\mathbb{B}}
\newcommand{\doubleC}{\mathbb{C}}
\newcommand{\doubleD}{\mathbb{D}}
\newcommand{\doubleE}{\mathbb{E}}
\newcommand{\doubleF}{\mathbb{F}}
\newcommand{\doubleG}{\mathbb{G}}
\newcommand{\doubleH}{\mathbb{H}}
\newcommand{\doubleI}{\mathbb{I}}
\newcommand{\doubleJ}{\mathbb{J}}
\newcommand{\doubleK}{\mathbb{K}}
\newcommand{\doubleL}{\mathbb{L}}
\newcommand{\doubleM}{\mathbb{M}}
\newcommand{\doubleN}{\mathbb{N}}
\newcommand{\doubleO}{\mathbb{O}}
\newcommand{\doubleP}{\mathbb{P}}
\newcommand{\doubleQ}{\mathbb{Q}}
\newcommand{\doubleR}{\mathbb{R}}
\newcommand{\doubleS}{\mathbb{S}}
\newcommand{\doubleT}{\mathbb{T}}
\newcommand{\doubleU}{\mathbb{U}}
\newcommand{\doubleV}{\mathbb{V}}
\newcommand{\doubleW}{\mathbb{W}}
\newcommand{\doubleX}{\mathbb{X}}
\newcommand{\doubleY}{\mathbb{Y}}
\newcommand{\doubleZ}{\mathbb{Z}}

% mathcal shorthands
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

% mathcalbar shorthands
\newcommand{\Acalbar}{\bar{\mathcal{A}}}
\newcommand{\Bcalbar}{\bar{\mathcal{B}}}
\newcommand{\Ccalbar}{\bar{\mathcal{C}}}
\newcommand{\Dcalbar}{\bar{\mathcal{D}}}
\newcommand{\Ecalbar}{\bar{\mathcal{E}}}
\newcommand{\Fcalbar}{\bar{\mathcal{F}}}
\newcommand{\Gcalbar}{\bar{\mathcal{G}}}
\newcommand{\Hcalbar}{\bar{\mathcal{H}}}
\newcommand{\Icalbar}{\bar{\mathcal{I}}}
\newcommand{\Jcalbar}{\bar{\mathcal{J}}}
\newcommand{\Kcalbar}{\bar{\mathcal{K}}}
\newcommand{\Lcalbar}{\bar{\mathcal{L}}}
\newcommand{\Mcalbar}{\bar{\mathcal{M}}}
\newcommand{\Ncalbar}{\bar{\mathcal{N}}}
\newcommand{\Ocalbar}{\bar{\mathcal{O}}}
\newcommand{\Pcalbar}{\bar{\mathcal{P}}}
\newcommand{\Qcalbar}{\bar{\mathcal{Q}}}
\newcommand{\Rcalbar}{\bar{\mathcal{R}}}
\newcommand{\Scalbar}{\bar{\mathcal{S}}}
\newcommand{\Tcalbar}{\bar{\mathcal{T}}}
\newcommand{\Ucalbar}{\bar{\mathcal{U}}}
\newcommand{\Vcalbar}{\bar{\mathcal{V}}}
\newcommand{\Wcalbar}{\bar{\mathcal{W}}}
\newcommand{\Xcalbar}{\bar{\mathcal{X}}}
\newcommand{\Ycalbar}{\bar{\mathcal{Y}}}
\newcommand{\Zcalbar}{\bar{\mathcal{Z}}}
% mathcalhat shorthands
\newcommand{\Acalhat}{\hat{\mathcal{A}}}
\newcommand{\Bcalhat}{\hat{\mathcal{B}}}
\newcommand{\Ccalhat}{\hat{\mathcal{C}}}
\newcommand{\Dcalhat}{\hat{\mathcal{D}}}
\newcommand{\Ecalhat}{\hat{\mathcal{E}}}
\newcommand{\Fcalhat}{\hat{\mathcal{F}}}
\newcommand{\Gcalhat}{\hat{\mathcal{G}}}
\newcommand{\Hcalhat}{\hat{\mathcal{H}}}
\newcommand{\Icalhat}{\hat{\mathcal{I}}}
\newcommand{\Jcalhat}{\hat{\mathcal{J}}}
\newcommand{\Kcalhat}{\hat{\mathcal{K}}}
\newcommand{\Lcalhat}{\hat{\mathcal{L}}}
\newcommand{\Mcalhat}{\hat{\mathcal{M}}}
\newcommand{\Ncalhat}{\hat{\mathcal{N}}}
\newcommand{\Ocalhat}{\hat{\mathcal{O}}}
\newcommand{\Pcalhat}{\hat{\mathcal{P}}}
\newcommand{\Qcalhat}{\hat{\mathcal{Q}}}
\newcommand{\Rcalhat}{\hat{\mathcal{R}}}
\newcommand{\Scalhat}{\hat{\mathcal{S}}}
\newcommand{\Tcalhat}{\hat{\mathcal{T}}}
\newcommand{\Ucalhat}{\hat{\mathcal{U}}}
\newcommand{\Vcalhat}{\hat{\mathcal{V}}}
\newcommand{\Wcalhat}{\hat{\mathcal{W}}}
\newcommand{\Xcalhat}{\hat{\mathcal{X}}}
\newcommand{\Ycalhat}{\hat{\mathcal{Y}}}
\newcommand{\Zcalhat}{\hat{\mathcal{Z}}}

% mathcaltil shorthands
\newcommand{\Acaltil}{\tilde{\mathcal{A}}}
\newcommand{\Bcaltil}{\tilde{\mathcal{B}}}
\newcommand{\Ccaltil}{\tilde{\mathcal{C}}}
\newcommand{\Dcaltil}{\tilde{\mathcal{D}}}
\newcommand{\Ecaltil}{\tilde{\mathcal{E}}}
\newcommand{\Fcaltil}{\tilde{\mathcal{F}}}
\newcommand{\Gcaltil}{\tilde{\mathcal{G}}}
\newcommand{\Hcaltil}{\tilde{\mathcal{H}}}
\newcommand{\Icaltil}{\tilde{\mathcal{I}}}
\newcommand{\Jcaltil}{\tilde{\mathcal{J}}}
\newcommand{\Kcaltil}{\tilde{\mathcal{K}}}
\newcommand{\Lcaltil}{\tilde{\mathcal{L}}}
\newcommand{\Mcaltil}{\tilde{\mathcal{M}}}
\newcommand{\Ncaltil}{\tilde{\mathcal{N}}}
\newcommand{\Ocaltil}{\tilde{\mathcal{O}}}
\newcommand{\Pcaltil}{\tilde{\mathcal{P}}}
\newcommand{\Qcaltil}{\tilde{\mathcal{Q}}}
\newcommand{\Rcaltil}{\tilde{\mathcal{R}}}
\newcommand{\Scaltil}{\tilde{\mathcal{S}}}
\newcommand{\Tcaltil}{\tilde{\mathcal{T}}}
\newcommand{\Ucaltil}{\tilde{\mathcal{U}}}
\newcommand{\Vcaltil}{\tilde{\mathcal{V}}}
\newcommand{\Wcaltil}{\tilde{\mathcal{W}}}
\newcommand{\Xcaltil}{\tilde{\mathcal{X}}}
\newcommand{\Ycaltil}{\tilde{\mathcal{Y}}}
\newcommand{\Zcaltil}{\tilde{\mathcal{Z}}}

% mathfrak shorthands
\newcommand{\Afrak}{\mathfrak{A}}
\newcommand{\Bfrak}{\mathfrak{B}}
\newcommand{\Cfrak}{\mathfrak{C}}
\newcommand{\Dfrak}{\mathfrak{D}}
\newcommand{\Efrak}{\mathfrak{E}}
\newcommand{\Ffrak}{\mathfrak{F}}
\newcommand{\Gfrak}{\mathfrak{G}}
\newcommand{\Hfrak}{\mathfrak{H}}
\newcommand{\Ifrak}{\mathfrak{I}}
\newcommand{\Jfrak}{\mathfrak{J}}
\newcommand{\Kfrak}{\mathfrak{K}}
\newcommand{\Lfrak}{\mathfrak{L}}
\newcommand{\Mfrak}{\mathfrak{M}}
\newcommand{\Nfrak}{\mathfrak{N}}
\newcommand{\Ofrak}{\mathfrak{O}}
\newcommand{\Pfrak}{\mathfrak{P}}
\newcommand{\Qfrak}{\mathfrak{Q}}
\newcommand{\Rfrak}{\mathfrak{R}}
\newcommand{\Sfrak}{\mathfrak{S}}
\newcommand{\Tfrak}{\mathfrak{T}}
\newcommand{\Ufrak}{\mathfrak{U}}
\newcommand{\Vfrak}{\mathfrak{V}}
\newcommand{\Wfrak}{\mathfrak{W}}
\newcommand{\Xfrak}{\mathfrak{X}}
\newcommand{\Yfrak}{\mathfrak{Y}}
\newcommand{\Zfrak}{\mathfrak{Z}}

% mathfrak shorthands
\newcommand{\Afrakbar}{\bar{\mathfrak{A}}}
\newcommand{\Bfrakbar}{\bar{\mathfrak{B}}}
\newcommand{\Cfrakbar}{\bar{\mathfrak{C}}}
\newcommand{\Dfrakbar}{\bar{\mathfrak{D}}}
\newcommand{\Efrakbar}{\bar{\mathfrak{E}}}
\newcommand{\Ffrakbar}{\bar{\mathfrak{F}}}
\newcommand{\Gfrakbar}{\bar{\mathfrak{G}}}
\newcommand{\Hfrakbar}{\bar{\mathfrak{H}}}
\newcommand{\Ifrakbar}{\bar{\mathfrak{I}}}
\newcommand{\Jfrakbar}{\bar{\mathfrak{J}}}
\newcommand{\Kfrakbar}{\bar{\mathfrak{K}}}
\newcommand{\Lfrakbar}{\bar{\mathfrak{L}}}
\newcommand{\Mfrakbar}{\bar{\mathfrak{M}}}
\newcommand{\Nfrakbar}{\bar{\mathfrak{N}}}
\newcommand{\Ofrakbar}{\bar{\mathfrak{O}}}
\newcommand{\Pfrakbar}{\bar{\mathfrak{P}}}
\newcommand{\Qfrakbar}{\bar{\mathfrak{Q}}}
\newcommand{\Rfrakbar}{\bar{\mathfrak{R}}}
\newcommand{\Sfrakbar}{\bar{\mathfrak{S}}}
\newcommand{\Tfrakbar}{\bar{\mathfrak{T}}}
\newcommand{\Ufrakbar}{\bar{\mathfrak{U}}}
\newcommand{\Vfrakbar}{\bar{\mathfrak{V}}}
\newcommand{\Wfrakbar}{\bar{\mathfrak{W}}}
\newcommand{\Xfrakbar}{\bar{\mathfrak{X}}}
\newcommand{\Yfrakbar}{\bar{\mathfrak{Y}}}
\newcommand{\Zfrakbar}{\bar{\mathfrak{Z}}}


% brackets
\newcommand{\rbr}[1]{\left( #1 \right)}
\newcommand{\rbrinline}[1]{( #1 )}
\newcommand{\cbr}[1]{\left\{ #1 \right\}}
\newcommand{\cbrinline}[1]{\{ #1 \}}
\newcommand{\sbr}[1]{\left[ #1 \right]}
\newcommand{\sbrinline}[1]{[ #1 ]}
\newcommand{\abr}[1]{\left\langle #1 \right\rangle}
\newcommand{\abrinline}[1]{\langle #1 \rangle}

% math
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\norminline}[1]{\| #1 \|}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\absinline}[1]{| #1 |}
\newcommand{\myset}[2]{\cbr{ #1 \,:\, #2 }}
\newcommand{\mysetinline}[2]{\cbrinline{ #1 \,:\, #2 }}
\newcommand{\mysetbar}[2]{\cbr{ #1 \,\middle|\, #2 }}
\newcommand{\mysetbarinline}[2]{\cbrinline{ #1 \,|\, #2 }}

\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}

\newcommand{\maximize}{\mathop{\mathrm{maximize}\;}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}\;}}

\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\supp}{\mathop{\mathrm{supp}}}
\newcommand{\spann}{\mathop{\mathrm{span}}}
\newcommand{\drm}{\mathrm{d}}

%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}{Lemma}
\numberwithin{lemma}{section}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}{Proposition}
\numberwithin{proposition}{section}
\fi

\ifx\corollary\undefined
  \newtheorem{corollary}{Corollary}
\numberwithin{corollary}{section}
\fi

\ifx\remark\undefined
\newtheorem{remark}{Remark}
\numberwithin{remark}{section}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\numberwithin{definition}{section}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\numberwithin{assumption}{section}
\fi

\ifx\problem\undefined
\newtheorem{problem}{Problem}
\numberwithin{problem}{section}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\numberwithin{example}{section}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\numberwithin{property}{section}
\fi

\ifx\remark\undefined
\newtheorem{observation}{Observation}
\numberwithin{observation}{section}
\fi


%---- Ide
\usepackage{bm}


\def\ci{\perp\!\!\!\perp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\trace}{Tr}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\vectorize}{vec}
\DeclareMathOperator{\MLP}{MLP}
\DeclareMathOperator{\LSTM}{LSTM}
\DeclareMathOperator{\Cell}{Cell}
\DeclareMathOperator{\FC}{FC}
\DeclareMathOperator{\Linear}{Linear}
\DeclareMathOperator{\sLSTM}{sLSTM}
\DeclareMathOperator{\Softmax}{Softmax}
\DeclareMathOperator{\GCN}{GCN}
\DeclareMathOperator{\ReLU}{ReLU}
%
\newcommand{\hata}{\hat{a}}
\newcommand{\hatb}{\hat{b}}
\newcommand{\hatc}{\hat{c}}
\newcommand{\hatd}{\hat{d}}
\newcommand{\hate}{\hat{e}}
\newcommand{\hatf}{\hat{f}}
\newcommand{\hatg}{\hat{g}}
\newcommand{\hath}{\hat{h}}
\newcommand{\hati}{\hat{i}}
\newcommand{\hatj}{\hat{j}}
\newcommand{\hatk}{\hat{k}}
\newcommand{\hatl}{\hat{l}}
\newcommand{\hatm}{\hat{m}}
\newcommand{\hatn}{\hat{n}}
\newcommand{\hato}{\hat{o}}
\newcommand{\hatp}{\hat{p}}
\newcommand{\hatq}{\hat{q}}
\newcommand{\hatr}{\hat{r}}
\newcommand{\hats}{\hat{s}}
\newcommand{\hatt}{\hat{t}}
\newcommand{\hatu}{\hat{u}}
\newcommand{\hatv}{\hat{v}}
\newcommand{\hatw}{\hat{w}}
\newcommand{\hatx}{\hat{x}}
\newcommand{\haty}{\hat{y}}
\newcommand{\hatz}{\hat{z}}
%
\newcommand{\bma}{\bm{a}}
\newcommand{\bmb}{\bm{b}}
\newcommand{\bmc}{\bm{c}}
\newcommand{\bmd}{\bm{d}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bmg}{\bm{g}}
\newcommand{\bmh}{\bm{h}}
\newcommand{\bmi}{\bm{i}}
\newcommand{\bmj}{\bm{j}}
\newcommand{\bmk}{\bm{k}}
\newcommand{\bml}{\bm{l}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bmn}{\bm{n}}
\newcommand{\bmo}{\bm{o}}
\newcommand{\bmp}{\bm{p}}
\newcommand{\bmq}{\bm{q}}
\newcommand{\bmr}{\bm{r}}
\newcommand{\bms}{\bm{s}}
\newcommand{\bmt}{\bm{t}}
\newcommand{\bmu}{\bm{u}}
\newcommand{\bmv}{\bm{v}}
\newcommand{\bmw}{\bm{w}}
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmy}{\bm{y}}
\newcommand{\bmz}{\bm{z}}
%
\newcommand{\rma}{\mathrm{a}}
\newcommand{\rmb}{\mathrm{b}}
\newcommand{\rmc}{\mathrm{c}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmf}{\mathrm{f}}
\newcommand{\rmg}{\mathrm{g}}
\newcommand{\rmh}{\mathrm{h}}
\newcommand{\rmi}{\mathrm{i}}
\newcommand{\rmj}{\mathrm{j}}
\newcommand{\rmk}{\mathrm{k}}
\newcommand{\rml}{\mathrm{l}}
\newcommand{\rmm}{\mathrm{m}}
\newcommand{\rmn}{\mathrm{n}}
\newcommand{\rmo}{\mathrm{o}}
\newcommand{\rmp}{\mathrm{p}}
\newcommand{\rmq}{\mathrm{q}}
\newcommand{\rmr}{\mathrm{r}}
\newcommand{\rms}{\mathrm{s}}
\newcommand{\rmt}{\mathrm{t}}
\newcommand{\rmu}{\mathrm{u}}
\newcommand{\rmv}{\mathrm{v}}
\newcommand{\rmw}{\mathrm{w}}
\newcommand{\rmx}{\mathrm{x}}
\newcommand{\rmy}{\mathrm{y}}
\newcommand{\rmz}{\mathrm{z}}
%
\newcommand{\bmA}{\bm{A}}
\newcommand{\bmB}{\bm{B}}
\newcommand{\bmC}{\bm{C}}
\newcommand{\bmD}{\bm{D}}
\newcommand{\bmE}{\bm{E}}
\newcommand{\bmF}{\bm{F}}
\newcommand{\bmG}{\bm{G}}
\newcommand{\bmH}{\bm{H}}
\newcommand{\bmI}{\bm{I}}
\newcommand{\bmJ}{\bm{J}}
\newcommand{\bmK}{\bm{K}}
\newcommand{\bmL}{\bm{L}}
\newcommand{\bmM}{\bm{M}}
\newcommand{\bmN}{\bm{N}}
\newcommand{\bmO}{\bm{O}}
\newcommand{\bmP}{\bm{P}}
\newcommand{\bmQ}{\bm{Q}}
\newcommand{\bmR}{\bm{R}}
\newcommand{\bmS}{\bm{S}}
\newcommand{\bmT}{\bm{T}}
\newcommand{\bmU}{\bm{U}}
\newcommand{\bmV}{\bm{V}}
\newcommand{\bmW}{\bm{W}}
\newcommand{\bmX}{\bm{X}}
\newcommand{\bmY}{\bm{Y}}
\newcommand{\bmZ}{\bm{Z}}
%
\newcommand{\bmzero}{\bm{0}}
\newcommand{\bmone}{\bm{1}}
\newcommand{\sfzero}{\mathsf{0}}
%
\newcommand{\bmalpha}{\bm{\alpha}}
\newcommand{\bmbeta}{\bm{\beta}}
\newcommand{\bmgamma}{\bm{\gamma}}
\newcommand{\bmdelta}{\bm{\delta}}
\newcommand{\bmepsilon}{\bm{\epsilon}}
\newcommand{\bmzeta}{\bm{\zeta}}
\newcommand{\bmeta}{\bm{\eta}}
\newcommand{\bmtheta}{\bm{\theta}}
\newcommand{\bmkappa}{\bm{\kappa}}
\newcommand{\bmlambda}{\bm{\lambda}}
\newcommand{\bmmu}{\bm{\mu}}
\newcommand{\bmnu}{\bm{\nu}}
\newcommand{\bmxi}{\bm{\xi}}
\newcommand{\bmpi}{\bm{\pi}}
\newcommand{\bmrho}{\bm{\rho}}
\newcommand{\bmsigma}{\bm{\sigma}}
\newcommand{\bmtau}{\bm{\tau}}
\newcommand{\bmphi}{\bm{\phi}}
\newcommand{\bmchi}{\bm{\chi}}
\newcommand{\bmpsi}{\bm{\psi}}
\newcommand{\bmomega}{\bm{\omega}}
%
\newcommand{\baralpha}{\bar{\alpha}}
\newcommand{\barbeta}{\bar{\beta}}
\newcommand{\bargamma}{\bar{\gamma}}
\newcommand{\bardelta}{\bar{\delta}}
\newcommand{\barepsilon}{\bar{\epsilon}}
\newcommand{\barzeta}{\bar{\zeta}}
\newcommand{\bareta}{\bar{\eta}}
\newcommand{\bartheta}{\bar{\theta}}
\newcommand{\barkappa}{\bar{\kappa}}
\newcommand{\barlambda}{\bar{\lambda}}
\newcommand{\barmu}{\bar{\mu}}
\newcommand{\barnu}{\bar{\nu}}
\newcommand{\barxi}{\bar{\xi}}
\newcommand{\barpi}{\bar{\pi}}
\newcommand{\barrho}{\bar{\rho}}
\newcommand{\barsigma}{\bar{\sigma}}
\newcommand{\bartau}{\bar{\tau}}
\newcommand{\barphi}{\bar{\phi}}
\newcommand{\barchi}{\bar{\chi}}
\newcommand{\barpsi}{\bar{\psi}}
\newcommand{\baromega}{\bar{\omega}}
%
\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}

\newcommand{\sfGamma}{\mathsf{\Gamma}}
\newcommand{\sfPsi}{\mathsf{\Psi}}
\newcommand{\sfPhi}{\mathsf{\Phi}}
\newcommand{\sfLambda}{\mathsf{\Lambda}}
\newcommand{\sfDelta}{\mathsf{\Delta}}
\newcommand{\sfSigma}{\mathsf{\Sigma}}
\newcommand{\sfOmega}{\mathsf{\Omega}}
\newcommand{\sfXi}{\mathsf{\Xi}}
%
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}
%
%
\newcommand{\bmcalA}{\bm{\mathcal{A}}}
\newcommand{\bmcalB}{\bm{\mathcal{B}}}
\newcommand{\bmcalC}{\bm{\mathcal{C}}}
\newcommand{\bmcalD}{\bm{\mathcal{D}}}
\newcommand{\bmcalE}{\bm{\mathcal{E}}}
\newcommand{\bmcalF}{\bm{\mathcal{F}}}
\newcommand{\bmcalG}{\bm{\mathcal{G}}}
\newcommand{\bmcalH}{\bm{\mathcal{H}}}
\newcommand{\bmcalI}{\bm{\mathcal{I}}}
\newcommand{\bmcalJ}{\bm{\mathcal{J}}}
\newcommand{\bmcalK}{\bm{\mathcal{K}}}
\newcommand{\bmcalL}{\bm{\mathcal{L}}}
\newcommand{\bmcalM}{\bm{\mathcal{M}}}
\newcommand{\bmcalN}{\bm{\mathcal{N}}}
\newcommand{\bmcalO}{\bm{\mathcal{O}}}
\newcommand{\bmcalP}{\bm{\mathcal{P}}}
\newcommand{\bmcalQ}{\bm{\mathcal{Q}}}
\newcommand{\bmcalR}{\bm{\mathcal{R}}}
\newcommand{\bmcalS}{\bm{\mathcal{S}}}
\newcommand{\bmcalT}{\bm{\mathcal{T}}}
\newcommand{\bmcalU}{\bm{\mathcal{U}}}
\newcommand{\bmcalV}{\bm{\mathcal{V}}}
\newcommand{\bmcalW}{\bm{\mathcal{W}}}
\newcommand{\bmcalX}{\bm{\mathcal{X}}}
\newcommand{\bmcalY}{\bm{\mathcal{Y}}}
\newcommand{\bmcalZ}{\bm{\mathcal{Z}}}

==> wsc25style.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% File contains:
%   fancyhdr.sty
%   psfig.sty
%   url.sty
%   wsc.bst
%   wscpaperproc.cls
%   wscsetup.sty
%   wsc.sty
%   wscbib.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



